Sampling Multimodal Distributions with the Vanilla Score: Benefits of Data-Based Initialization

There is a long history, as well as a recent explosion of interest, in statistical and generative modeling approaches based on score functions -- derivatives of the log-likelihood of a distribution. In seminal works, Hyv\"arinen proposed vanilla score matching as a way to learn distributions from data by computing an estimate of the score function of the underlying ground truth, and established connections between this method and established techniques like Contrastive Divergence and Pseudolikelihood estimation. It is by now well-known that vanilla score matching has significant difficulties learning multimodal distributions. Although there are various ways to overcome this difficulty, the following question has remained unanswered -- is there a natural way to sample multimodal distributions using just the vanilla score? Inspired by a long line of related experimental works, we prove that the Langevin diffusion with early stopping, initialized at the empirical distribution, and run on a score function estimated from data successfully generates natural multimodal distributions (mixtures of log-concave distributions).

==> helper.tex <==
\section{Auxiliary lemmas}
\begin{proposition} \label{prop:composite of exponential and polynomial terms}
For any constant $a > 0, b, p\in \N_{\geq 0}$
$f(x) = \exp (-a x - b)  x^p$ is decreasing on $[p/a, +\infty)$ 
\end{proposition}
\begin{proof}
Let $g(x) = \log f(x) = -ax- b + p \log x$ and observe that
\[g'(x) = -a + p/x  \leq 0 \] when $ x \geq p/a$, so the claim follows by integrating. 
\end{proof}

\begin{proposition}\label{prop:tv distance mixture bound}
Let $P_1, \dots, P_k, Q_1, \dots, Q_k$ be distributions s.t. $d_{TV} (P_i, Q_i) \leq \epsilon_i.$
Let $\alpha_1, \cdots, \alpha_k, \beta_1, \cdots, \beta_k$ be s.t. $\alpha_i, \beta_i \geq 0\forall i$ and $\sum_i \alpha_i = \sum_i \beta_i = 1.$  Then
\[d_{TV}(\sum_i \alpha_i P_i, \sum_i \alpha_i Q_i) \leq \sum_i \alpha_i \epsilon_i \]
and
\[d_{TV}(\sum_i \alpha_i Q_i, \sum_i \beta_i Q_i)\leq \frac{1}{2} \sum_{i} \abs{\alpha_i -\beta_i} \]
\end{proposition}
\begin{proof}
By triangle inequality
\begin{align*}
  2 d_{TV} (\sum_i \alpha_i P_i, \sum_i \alpha_i Q_i) &=
\int_{x\in \Omega} \abs{\sum_{i} \alpha_i P_i(x) - \sum_i \alpha_i Q_i(x)} dx \\
&\leq \int_{x\in \Omega}\sum_{i} \alpha_i \abs{P_i(x) -Q_i(x)} dx = 2\sum_{i} \alpha_i  d_{TV}(P_i, Q_i)
\end{align*}
Similarly,
\begin{align*}
  2 d_{TV} (\sum_i \alpha_i Q_i, \sum_i \beta_i Q_i) &=
\int_{x\in \Omega} \abs{\sum_{i} \alpha_i Q_i(x) - \sum_i \beta_i Q_i(x)} dx \\
&\leq \int_{x\in \Omega}\sum_{i}\abs{ \alpha_i-\beta_i}  Q_i(x) dx =\sum_{i} \abs{\alpha_i -\beta_i}
\end{align*}
\end{proof}

\begin{proposition} \label{prop:init partition bound} Suppose $\mu = \sum_{i\in I} p_i \mu_i$ with $ I$
Fix a set $C\subseteq I.$
If the overlap between $\mu_i,\mu_j$ for $i\in C$ and $j\not \in C$ is $\leq \delta'$ for all such $i,j$ then
\[\mu(\set{x: i_{\max}(x) \in C})\geq p_C (1-\delta'\abs{I})  % (1-\delta' |I|) \max_{i\in C} p_i 
\] 
\end{proposition}
To remove dependency on $p_*,$ we will use the following modified version of \cref{prop:init partition bound}
\begin{proposition}\label{prop:init partition bound modified}
   Fix $C,C_*\subseteq I$ s.t. $ C\cap C_*=\emptyset.$ Let $I' = I\setminus C_*.$ If for $i\in C, j\in I'\setminus C,$ the overlap between $\mu_i $ and $\mu_j$ is $\leq \delta'$ then for $i_{\max, I'} (x) =\arg\max_{i\in I'} \mu_i(x)$
   \[\mu_I (\set{x: i_{\max, I'} (x) \in C })\geq p_C (1-\delta' \abs{I}) \] 
\end{proposition}
\begin{proof}[Proof of \cref{prop:init partition bound,prop:init partition bound modified}]
We first prove \cref{prop:init partition bound}.
For $i\in C,j\not \in C$
\begin{align*}
  \mu_i(\set{x: \mu_i(x) \leq \mu_j(x) }) &= \int_{x: \mu_i(x) \leq \mu_j(x) }\mu_i(x) dx \\
  &= \int_{x: \mu_i(x) \leq \mu_j(x) } \min \set{\mu_i(x), \mu_j(x)} dx  \\
  &\leq \int \min \set{\mu_i(x), \mu_j(x)}  dx  \leq \delta'   
\end{align*}
By union bound, for $i\in C$
\[\mu_i( \set{x | \exists j\not \in C: \mu_i(x) \leq \mu_j(x) }) \leq \delta' \abs{I}\]
Let $\Lambda =\set{x: i_{\max}(x) \in C}  . $
%Let $i=\arg\max_{i'\in C} p_i.$ 
If $ \forall j \not\in C: \mu_i(x) > \mu_j(x)$ then $ i_{\max}(x) \in C.$ Thus $\Lambda_i :=\set{x: \mu_i(x) > \mu_j(x) \forall j\not\in C }\subseteq\Lambda $
and $\mu_i(\Lambda_i) = 1- \mu_i(\set{x \lvert \exists j\not\in C : \mu_i(x) \leq \mu_j(x)} \geq 1-\delta'\abs{I}.$ Since $\mu(x) \geq \sum_{i\in C} p_i \mu_i(x)$
\begin{align*}
    \mu(\set{x:i_{\max}(x)\in C}) &= \int_{x\in \Lambda} \mu(x) dx \geq \int_{x\in \Lambda} \sum_{i\in C} p_i\mu_i(x) dx = \sum_{i\in C}p_i \mu_i(\Lambda) \\
    &\geq \sum_{i\in C}p_i\mu_i(\Lambda_i) \geq\sum_{i\in C} p_i (1-\delta'\abs{I})= p_C (1-\delta'\abs{I}) 
\end{align*}
%\[\mu(\set{x:i_{\max}(x)\in C}) \geq p_i \mu_i(\set{x: i_{\max}(x)\in C}) \geq p_i\mu_i(\set{x | \forall j\not \in C: \mu_i(x) \geq \mu_j(x) }) \geq p_i (1-\delta'|I|).\]

The proof of \cref{prop:init partition bound modified} is identical, except we will consider $i\in C,j\in I'\setminus C$ and argue that $ \mu_i({x: \mu_i(x) \leq\mu_j(x)}) \leq \delta'.$ Then $ \mu_i({x\lvert \exists j\in I'\setminus C: \mu_i(x)\leq \mu_j(x) })\leq \delta'\abs{I}.$ For $i\in C,$ $\Lambda_i = \set{x\lvert \mu_i(x) >\mu_j(x) \forall j\in I'\setminus C}$ then $ \mu_i(\Lambda_i) \geq 1 - \delta'\abs{I}$ and $\Lambda_i \subseteq \set{x:i_{\max, I'}(x)\in C}.$ Finally,
\[\mu (\set{x: i_{\max, I'}(x) \in  C})\geq \sum_{i\in C} p_i \mu_i(\Lambda_i) \geq p_C (1 - \delta'\abs{I}). \]

\end{proof}
We need this proposition to go from \cref{lem:well separated cluster} to \cref{thm:continuous mixing}
\begin{comment}
\begin{proposition}\label{prop:process init from sample disjoint case}
For $x\in \R^d,$ let $ (X_t^x)_t$ be a process initialized at $\delta_x.$
Suppose there exists $T> 0, \epsilon_{TV}\in (0,1), \epsilon_{\text{sample}}\in (0,p_*/10) $ and a partition of $I$ into $C_1, \dots, C_m$ s.t. %s.t. for each $S\in \set{C_1, \dots, C_m},$ 
\[\P_{x\sim\mu}[d_{TV} (X_{T}^x , \mu_{C_{\max}(x)} ) \leq \epsilon_{TV}/2] \geq 1-\epsilon_{\text{sample}} \]
where $C_{\max}(x)$ is the unique part $C_r$ containing $i_{\max}(x)=\arg\max_{i}\mu_i(x). $
In addition, there exists $\delta'\in (0, \tilde{\epsilon}_{TV})$ s.t. for $C \in \set{C_1, \dots, C_m}$
\[\P_{x\sim\mu}[ C_{\max}(x) = C]\geq p_C (1-\delta').\]
%Suppose $ \epsilon_{\text{sample}} \leq  p_*/10.$
Let $U_{\text{sample}}$ be a set of $M$ i.i.d. samples from $\mu$ and $ \nu_{\text{sample}}$ be the uniform distribution over  $U_{\text{sample}}.$
Let $(X_{nh}^{\nu_{\text{sample}}})_{t\geq 0 }$ be the process with score estimate $s$ initialized at $\nu_{\text{sample}}.$
With probability $\geq 1 - \abs{I} \exp(- p_* M \epsilon_{\text{sample}}^2/6)$
\[d_{TV} (X_{T}^{\nu_{\text{sample}}}, \mu) \leq  \epsilon_{TV}  + 3\abs{I}^2 \epsilon_{\text{sample}}\]%\epsilon_{TV} + 2\abs{I} \delta' + 3\abs{I}^2 \epsilon_{\text{sample}} \leq  \epsilon_{TV} +  \]
Thus, letting $\epsilon_{\text{sample}} = p_*\epsilon_{TV}/(6\abs{I}^2),$ and $M = 8p_*^{-3} \epsilon_{TV}^{-2} (\log (\abs{I} \epsilon_{\text{sample}}^{-1}) ) $ we have, with probability $ \geq  1- \epsilon_{\text{sample}}$ over $U_{\text{sample}},$ let $\hat{\mu} = \mathcal{L}(X_{T}^{\nu_{\text{sample}}} | U_{\text{sample}})$,
\[d_{TV}(\hat{\mu}, \mu) \leq \epsilon_{TV} \]

\end{proposition}
\end{comment}
\begin{proposition}\label{prop:process init from sample disjoint case}
Consider distributions $\mu_i$ for $i\in I.$ Suppose $\mu = \sum_{i\in I} p_i \mu_i$ for $p_i> 0$ and $\sum_{i\in I }p_i =1.$ Suppose we have a partition $\mathcal{C}$ of $I$ into $C_1, \dots, C_m$. For $x\in \R^d,$ let $C= C_{\max}(x)$ be the unique part of the partition $\mathcal{C}$ containing $i_{\max}(x)=\arg\max_{i\in I}\mu_i(x). $
Let $p_* =\min_{i\in I} p_i.$
For $x\in \R^d,$ let $ (X_t^x)_t$ be a process initialized at $\delta_x.$ 
Suppose for any $\tilde{\epsilon}_{TV}\in (0,1/10), \tilde{\epsilon}_{\text{sample}}\in (0,p_*/3) ,$ there exists $T_{\tilde{\epsilon}_{TV}, \tilde{\epsilon}_{\text{sample}}}$ such that the following holds: %For $x\sim \mu,$then
\[\P_{x\sim \mu} [d_{TV}(\mathcal{L}(X_{T_{\tilde{\epsilon}_{TV}, \tilde{\epsilon}_{\text{sample}}}}^x |x)  ,\mu_{C_{\max}(x)}) \leq \tilde{\epsilon}_{TV}] \geq 1-\tilde{\epsilon}_{\text{sample}} .\]

In addition, there exists $\delta'\in (0, \tilde{\epsilon}_{TV})$ s.t. for $C \in \set{C_1, \dots, C_m}$
\[\P_{x\sim\mu}[ C_{\max}(x) = C]\geq p_C (1-\delta').\]
%Suppose $ \epsilon_{\text{sample}} \leq  p_*/10.$
Let $U_{\text{sample}}$ be a set of $M$ i.i.d. samples from $\mu$ and $ \nu_{\text{sample}}$ be the uniform distribution over  $U_{\text{sample}}.$
Let $(X_{t}^{U_{\text{sample}}})_{t\geq 0 }$ be the process with score estimate $s$ initialized at $\nu_{\text{sample}}.$
If $M \geq  6\times 10^2 \abs{I}^2 \epsilon_{TV}^{-2} p_*^{-1} \log (\abs{I} \epsilon_{\text{sample}}^{-1}),$
with probability $ \geq  1- \epsilon_{\text{sample}}$ over $U_{\text{sample}},$ let $T = T_{\frac{\epsilon_{TV}}{9\abs{I}},  \min \set{\frac{\epsilon_{TV}}{9\abs{I}^2 } , p_*/3} } $ and $\hat{\mu} = \mathcal{L}(X_{T}^{\nu_{\text{sample}}} | U_{\text{sample}})$, then
\[\P_{U_{\text{sample}} } [d_{TV}( \mathcal{L}(X_{T}^{U_{\text{sample}}} | U_{\text{sample}}), \mu) \leq \epsilon_{TV} ] \geq 1- \epsilon_{\text{sample}} \]
\end{proposition}
To remove the dependency on $p_*=\min_{i\in I} p_i$, we will use this modified version of \cref{prop:process init from sample disjoint case}.
\begin{proposition}\label{prop:process init from sample disjoint case modified}
Consider distributions $\mu_i$ for $i\in I.$ Suppose $\mu = \sum_{i\in I} p_i \mu_i$ for $p_i> 0$ and $\sum_{i\in I }p_i =1.$ %Suppose we have $C_*\subseteq I$ and a partition $I' = I\setminus C_*$
For $x\in \R^d,$ let $ (X_t^x)_t$ be a process initialized at $\delta_x.$ 
Suppose for any $\tilde{\epsilon}_{TV}\in (0,1/10), \tilde{\epsilon}_{\text{sample}}\in (0,1) $, there exists $T_{\tilde{\epsilon}_{TV}, \tilde{\epsilon}_{\text{sample}}}$ such that the following holds. Let $I'=\set{i\in I: p_i \geq  \frac{\tilde{\epsilon}_{TV}}{\abs{I}}}$ and $C_* =C\setminus I'.$ Suppose we have a partition $\mathcal{C}$ of $I'$ into $C_1, \cdots, C_r .$ For $x\in \R^d,$ let $C_{\max}(x)$ be the unique part of the partition $\mathcal{C}$ containing $i_{\max,I'}(x)=\arg\max_{i\in I' }\mu_i(x). $

\[\P_{x\sim \mu} [d_{TV}(\mathcal{L}(X_{T_{\tilde{\epsilon}_{TV}, \tilde{\epsilon}_{\text{sample}}}}^x |x)  ,\mu_{C_{\max}(x) }) \leq \tilde{\epsilon}_{TV}] \geq 1-\tilde{\epsilon}_{\text{sample}} .\]
%s.t. for each $S\in \set{C_1, \dots, C_m},$ 
%\[\P_{x\sim\mu}[d_{TV} (X_{T}^x , \mu_{C_{\max}(x)} ) \leq \tilde{\epsilon}_{TV}] \geq 1-\tilde{\epsilon}_{\text{sample}} \]

In addition, there exists $\delta'\in (0, \tilde{\epsilon}_{TV})$ s.t. for $C \in \set{C_1, \dots, C_m}$
\[\P_{x\sim\mu}[ C_{\max, I'}(x) = C]\geq p_C (1-\delta').\]
%Suppose $ \epsilon_{\text{sample}} \leq  p_*/10.$
Let $U_{\text{sample}}$ be a set of $M$ i.i.d. samples from $\mu$ and $ \nu_{\text{sample}}$ be the uniform distribution over  $U_{\text{sample}}.$
Let $(X_{t}^{U_{\text{sample}}})_{t\geq 0 }$ be the process with score estimate $s$ initialized at $\nu_{\text{sample}}.$
% With probability $\geq 1 - \abs{I} \exp(- p_* M \epsilon_{\text{sample}}^2/6)$
% \[d_{TV} (X_{T}^{\nu_{\text{sample}}}, \mu) \leq  \epsilon_{TV}  + 3\abs{I}^2 \epsilon_{\text{sample}}\]%\epsilon_{TV} + 2\abs{I} \delta' + 3\abs{I}^2 \epsilon_{\text{sample}} \leq  \epsilon_{TV} +  \]
% Thus, letting $\epsilon_{\text{sample}} = p_*\epsilon_{TV}/(6\abs{I}^2),$ and $M = 8p_*^{-3} \epsilon_{TV}^{-2} (\log (\abs{I} \epsilon_{\text{sample}}^{-1}) ) $ 
If $M \geq 2\times 10^4 \abs{I}^3 \epsilon_{TV}^{-3} \log (\abs{I} \epsilon_{\text{sample}}^{-1}),$ then
\[\P_{U_{\text{sample}} } [d_{TV}( \mathcal{L}(X_{T}^{U_{\text{sample}}} | U_{\text{sample}}), \mu) \leq \epsilon_{TV} ] \geq 1- \epsilon_{\text{sample}} \]
\end{proposition}
\begin{proof}[Proof of \cref{prop:process init from sample disjoint case} and \cref{prop:process init from sample disjoint case modified}]

We will prove \cref{prop:process init from sample disjoint case modified}. The proof of \cref{prop:process init from sample disjoint case} is similar. Set
 $\tilde{\epsilon}_{\text{sample}} = \frac{\tilde{\epsilon}_{TV}}{\abs{I}}. $
%Let $ J = \set{r: p_{i} \geq \frac{\tilde{\epsilon}_{TV}}{\abs{I}} \forall i \in C_r }.$
%For $r\in J,$
Let $ \Omega_r=\set{x: C_{\max}(x)=C_r \land  d_{TV} (X_{T}^x , \mu_{C_{\max}(x)} ) \leq \epsilon_{TV}}.$ Clearly, $\Omega_r$ are disjoint, and by union bound $\mu(\Omega_r) \geq \tilde{p}_{C_r}:= (1-\delta') p_{C_r} - \tilde{\epsilon}_{\text{sample}}\geq \frac{\tilde{\epsilon}_{TV} }{10 \abs{I}}.$

Let $ U_r = \Omega_r \cap U_{\text{sample}} $ then Chernoff bound gives
\[\P[\abs{U_r} \geq M \tilde{p}_{C_r} (1-\tilde{\epsilon}_{TV})   ]\geq 1- \exp(-\tilde{\epsilon}_{TV}^2 \tilde{p}_{C_r} M /2) \geq 1- \exp(-\frac{\tilde{\epsilon}_{TV}^3 M }{20 \abs{I} })  \]

Let $\mathcal{E}$ be the event $\forall r: \abs{U_r} \geq M \tilde{p}_{C_r} (1-\tilde{\epsilon}_{TV}).$ By union bound, $\P[\mathcal{E}] \geq 1- \abs{I} \exp(-\frac{\tilde{\epsilon}_{TV}^3 M }{20 \abs{I} }). $ 

Suppose $\mathcal{E}$ happens. 
Let $U_{\emptyset} =U_{\text{sample}} \setminus \bigcup_{r\in J}  U_{r} $ then 
\begin{align*}
 \abs{U_{\emptyset}} &\leq M - M (1-\tilde{\epsilon}_{TV}) \sum_{r\in J }( p_{C_r} (1- \delta') -  \frac{\tilde{\epsilon}_{TV}}{\abs{I}}) \\
 &\leq M\left[1- (1- \tilde{\epsilon}_{TV}) ( (1-\delta') (1-\tilde{\epsilon}_{TV}) -   \tilde{\epsilon}_{TV} ) \right]  \\
 &\leq M  ( 3 \tilde{\epsilon}_{TV} + \delta')    \leq 4 M \tilde{\epsilon}_{TV}
\end{align*}
where the second inequality is due to $ \sum_{r\in J} p_{C_r} \geq 1 - \sum_{r\not\in J} p_{C_r} \geq 1 - \abs{I}\times \tilde{\epsilon}_{TV}/\abs{I}.$

Note that $\mathcal{L}(X_T^{U_{\text{sample}}} | U_{\text{sample}}) = \frac{1}{M}  \sum_{x\in U_{\text{sample}}} \mathcal{L}(X_T^x |x ).$ %where $\mathcal{L}(X)$ refers to the law of the random variable $X.$
Thus, let $\hat{\mu} = \sum_{r} \frac{\abs{U_r}}{\abs{U_{\text{sample}}\setminus U_\emptyset }} \mu_{C_r}$ and $ \tilde{\mu} := \sum_{r} \frac{\abs{U_{r} }}{M} \mu_{C_r} + \frac{\abs{U_{\emptyset} }}{M}\hat{\mu}$,  we can apply part 1 of \cref{prop:tv distance mixture bound}
\begin{align*}
    d_{TV}(\mathcal{L}(X_T^{U_{\text{sample}}}| U_{\text{sample}}),  \tilde{\mu}) &\leq M^{-1} \left ( \sum_{r} \sum_{x\in U_{r}} d_{TV}(\mathcal{L}(X_T^x|x), \mu_{C_r}) + \sum_{x\in U_{\emptyset} } d_{TV} (\mathcal{L}(X_T^x|x), \hat{\mu})\right)\\
    &\leq M^{-1} (\tilde{\epsilon}_{TV} (M - \abs{U_{\emptyset}}) +   \abs{U_{\emptyset}}) \\
    &\leq \tilde{\epsilon}_{TV} + 4 \tilde{\epsilon}_{TV} \leq 5 \tilde{\epsilon}_{TV}
\end{align*}
Next, note that $\mu=\sum_{r} p_{C_r} \mu_{C_r} + p_{C_*}\mu_{C_*} $ and $\tilde{\mu} =\sum_{r}\bar{p}_{C_r} \mu_{C_r} $ with $\bar{p}_{C_r}  :=  \frac{\abs{U_r} }{M} (1+ \frac{\abs{U_{\emptyset} }}{ \abs{U_{\text{sample}}\setminus U_\emptyset }  } )  = \frac{\abs{U_r} }{M - \abs{U_{\emptyset}} }.$  We bound $\abs{\bar{p}_{C_r} - p_{C_r}}.$
\begin{align*}
    \frac{\abs{U_r} }{M - \abs{U_{\emptyset}} } \geq \frac{\abs{U_r}}{M}\geq \frac{M (1-\tilde{\epsilon}_{TV} )  ((1-\delta') p_{C_r} - \frac{\tilde{\epsilon}_{TV}}{\abs{I}} ) }{M  } \geq p_{C_r} (1 - \tilde{\epsilon}_{TV} - \delta') -\frac{\tilde{\epsilon}_{TV}}{\abs{I}} \geq p_{C_r} - \tilde{\epsilon}_{TV} (2 + \frac{1}{\abs{I}})
\end{align*}
We upper bound $\abs{U_r}.$ Since $U_r $'s are disjoint,
\begin{align*}
    \abs{U_r} \leq M - \sum_{s\in J, s\neq r}
    \abs{U_{s}} \leq M - M \sum_{s\in J, s\neq r} \left[ p_{C_s} (1 - \tilde{\epsilon}_{TV} - \delta') -\frac{\tilde{\epsilon}_{TV}}{\abs{I}} \right] \leq M (p_{C_r} + 3\tilde{\epsilon}_{TV}  +\delta' )\leq M (p_{C_r}+ 4 \tilde{\epsilon}_{TV} )
\end{align*}
where the first inequality is due to the lower bound of $\abs{U_s}$ above and the second inequality is due to $ 1-\sum_{s: s\neq r} p_{C_s} \leq p_{C_r} + \tilde{\epsilon}_{TV}$ and $ \sum_{s:s\neq r} p_{C_s}  (\tilde{\epsilon}_{TV} + \delta') \leq (\tilde{\epsilon}_{TV} + \delta') .$ Thus
\begin{align*}
    \frac{\abs{U_r} }{M - \abs{U_{\emptyset}} }  -p_{C_r}\leq \frac{M (p_{C_r} +4 \tilde{\epsilon}_{TV} ) }{M (1- 4 \tilde{\epsilon}_{TV} )} -p_{C_r} \leq \frac{4 \tilde{\epsilon}_{TV} (p_{C_r}+1) }{1-4 \tilde{\epsilon}_{TV} } \leq 16 \tilde{\epsilon}_{TV} 
\end{align*}
where in the last inequality, we use the bounds $ \tilde{\epsilon}_{TV}\leq 1/10$ and $p_{C_r}\leq 1.$
thus 
\[\abs{\bar{p}_{C_r} - p_{C_r} }\leq \max \set{  16 \tilde{\epsilon}_{TV} , \tilde{\epsilon}_{TV} (2 + \frac{1}{\abs{I}}) } \]
Part 2 of \cref{prop:tv distance mixture bound} gives
\begin{align*}
    2d_{TV}(\mu,\tilde{\mu}) \leq \sum_{r} \abs{\bar{p}_{C_r} - p_{C_r} } + p_{C_*} &\leq\abs{I}  \max \set{  16 \tilde{\epsilon}_{TV} , \tilde{\epsilon}_{TV} (2 + \frac{1}{\abs{I}}) }   + \abs{I}\times \tilde{\epsilon}_{TV}/\abs{I}\\
    &\leq (16\abs{I} +1)\tilde{\epsilon}_{TV}
\end{align*}
Thus by triangle inequality,
\[ d_{TV}(\mathcal{L}(X_T^{U_{\text{sample}}}| U_{\text{sample}}),  \mu) \leq  d_{TV}(\mathcal{L}(X_T^{\nu_{\text{sample}}}| U_{\text{sample}}),  \tilde{\mu}) + d_{TV}(\mu,\tilde{\mu})  \leq 9 \abs{I} \tilde{\epsilon}_{TV}\]
Letting $\tilde{\epsilon}_{TV}=\frac{\epsilon_{TV}}{9\abs{I}}$ and $M  \geq  2\times 10^4 \abs{I}^3 \epsilon_{TV}^{-3} \log (\abs{I} \epsilon_{\text{sample}}^{-1}) \geq  20 \abs{I} \tilde{\epsilon}_{TV}^{-3} \log (\abs{I} \epsilon_{\text{sample}}^{-1})   $ gives the desired result.
 
 In the proof of \cref{prop:process init from sample disjoint case} we will set $\tilde{\epsilon}_{\text{sample}} = \min\set{\frac{\tilde{\epsilon}_{TV}}{\abs{I}}, p_*/3}$ which implies $\mu(\Omega_r) \geq p_*/3$ and the event $\mathcal{E}$ happens with probability $ 1-\abs{I} \exp(-\frac{p_* \tilde{\epsilon}_{TV}^2 M}{6 }).$ The rest of the argument follows through, and we need to set $M = 6\times 10^2 p_*^{-1} |I|^2 \epsilon_{TV}^{-2} \log (\abs{I} \epsilon_{\text{sample}}^{-1} )  $ to ensure $\mathcal{E}$ happens with probability $\geq 1-\epsilon_{\text{sample}}. $
 
\end{proof}
\begin{comment}
\begin{proof}
Let $ \Omega_r=\set{x: C_{\max}(x)=C_r \land  d_{TV} (X_{T}^x , \mu_{C_{\max}(x)} ) \leq \epsilon_{TV}}.$ Clearly, $\Omega_r$ are disjoint, and by union bound $\mu(\Omega_r) \geq \tilde{p}_{C_r}:= (1-\delta') p_{C_r} - \epsilon_{\text{sample}} \geq p_*/3. $
Let $ U_r = \Omega_r \cap U_{\text{sample}} $ then Chernoff bound gives
\[\P[\abs{U_r} \geq \tilde{p}_{C_r} (1-\epsilon_{\text{sample}})   ]\geq 1- \exp(-\epsilon_{\text{sample}}^2 \tilde{p}_{C_r} M /2)  \]
Let $\mathcal{E}$ be the event $\forall r: \abs{U_r} \geq \tilde{p}_{C_r} (1-\epsilon_{\text{sample}}).$ By union bound, $\P[\mathcal{E}] \geq 1- \abs{I} \exp(- p_* M \epsilon_{\text{sample}}^2/6). $ Suppose $\mathcal{E}$ happens.

Let $U_{\emptyset} =U_{\text{sample}} \setminus \bigcup_{r}  U_{r} $ then $\abs{U_{\emptyset}} \leq M - M (1-\epsilon_{\text{sample}}) \sum_{r}( p_{C_r} (1- \delta') -  \epsilon_{\text{sample}}) \leq M(1- (1- \epsilon_{\text{sample}}) (1-\delta' - \abs{I} \epsilon_{\text{sample}} ) )  \leq M ((\abs{I}+1)\epsilon_{\text{sample}} + \delta').$

Since $U_r$'s are disjoint, 
\begin{align*}
  \abs{U_r}/M -(1-\epsilon_{\text{sample}}) \tilde{p}_{C_r}&\leq 
 1 -(1-\epsilon_{\text{sample}}) \sum_{r'} ((1-\delta') p_{C_{r'}} - \epsilon_{\text{sample}} ) \\
 &\leq \delta' + (\abs{I}+1)\epsilon_{\text{sample}}    
\end{align*}
Note that $\mathcal{L}(X_T^{\nu_0} | U_{\text{sample}}) = \frac{1}{M}  \sum_{x\in U_{\text{sample}}} \mathcal{L}(X_T^x |x )$ where $\mathcal{L}(X)$ refers to the law of the random variable $X.$ Thus, let $\hat{\mu} = \sum_{r\in J} \frac{\abs{U_r}}{\abs{U_{\text{sample}}\setminus U_\emptyset }} \mu_{C_r}$ and $ \tilde{\mu} := \sum_{r\in J} \frac{\abs{U_{r} }}{M} \mu_{C_r} + \frac{\abs{U_{\emptyset} }}{M}\hat{\mu}$,  we can apply part 1 of \cref{prop:tv distance mixture bound}
\begin{align*}
    d_{TV}(X_T^{\nu_0},  \tilde{\mu}) &\leq M^{-1} \left ( \sum_{r} \sum_{x\in U_{r}} d_{TV}(X_T^x, \mu_{C_r}) + \sum_{x\in U_{\emptyset} } d_{TV} (X_T^x, \hat{\mu})\right)\\
    &\leq M^{-1} (\epsilon_{TV} (M - \abs{U_{\emptyset}}) +   \abs{U_{\emptyset}}) \\
    &\leq  \epsilon_{TV} + (\abs{I} +1)\epsilon_{\text{sample}} + \delta'
\end{align*}
Next, note that $\mu=\sum_{r} p_{C_r} \mu_{C_r} $ and $\tilde{\mu} =\sum_{\hat{r}} (\frac{\abs{U_r} }{M} +  p_{C_r} \frac{\abs{U_{\emptyset} }}{M} ) \mu_{C_r} .$  Part 2 of \cref{prop:tv distance mixture bound} gives
\begin{align*}
   d_{TV}( \tilde{\mu}, \mu) &\leq \frac{1}{2} \sum_{r} \abs{p_{C_r} - (\frac{\abs{U_{r}} }{M} +  p_{C_r} \frac{\abs{U_{\emptyset} }}{M} ) } =  \frac{1}{2} \sum_{r} \abs{  p_{C_r} (1 - \frac{\abs{U_{\emptyset} }}{M} ) -\frac{\abs{U_{r}} }{M}  } \\
   &\leq \frac{1}{2} \sum_{r} \max \set{p_{C_r}  -  \frac{\abs{U_{r}} }{M} ,\frac{\abs{U_{r}} }{M}-  p_{C_r} (1-\epsilon_{\text{sample}} ) (1-\delta' - \abs{I} \epsilon_{\text{sample}}) }\\
   &\leq  \frac{1}{2} \sum_{r} \max \set{p_{C_r}    (\epsilon_{\text{sample}} +\delta') +\epsilon_{\text{sample}} , (2\abs{I} +1)\epsilon_{\text{sample}} + \delta'   } \\
   &\leq (2\abs{I}+1)\abs{I} \epsilon_{\text{sample}} +\abs{I} \delta'
\end{align*}
thus by triangle inequality, and use the fact that $ \delta'\abs{I} < \epsilon_{\text{sample}},$ we have
\[d_{TV} (X_T^{\nu_0}, \mu) \leq  d_{TV}(X_T^{\nu_0},  \tilde{\mu})  + d_{TV}( \tilde{\mu}, \mu) \leq \epsilon_{TV} + 3\abs{I}^2 \epsilon_{\text{sample}}   \]
\end{proof}
\end{comment}
%This proposition allows us to say if a certain process initialized at the uniform distribution over $M_0$ i.i.d. samples from $\mu$ converges to $\mu$ then if we increase the number of samples in the initial distribution, the .
This proposition is used in \cref{thm:discrete mixing for cluster of distribution with close centers} to go from a set of samples of fixed size $M_0$ to a set of samples with size $M $ that can be arbitrarily large.

\begin{proposition}\label{prop:boost small sample batch to big batch}
  Fix distributions $\mu_{\text{sample}}, \mu.$
    For a set $U_{\text{sample}}\subseteq \R^d$,  let $ (X_t^{U_{\text{sample}} })_t$ be a process initialized at $\nu_{\text{sample}},$ the uniform distribution over
    $U_{\text{sample}}.$
Suppose there exists $T> 0, \epsilon_{TV}\in (0,1)$ 
s.t. with probability $ \geq 1-\epsilon_{TV}/10$ over the choice of  $U_{\text{sample}}$ consisting of $M_0$ i.i.d. samples from $\mu_{\text{sample}} ,$  $d_{TV}(\mathcal{L} (X_T^{U_{\text{sample}} } | U_{\text{sample}}), \mu) \leq \epsilon_{TV}/10.$
Then, for $M \geq  6 \epsilon_{TV}^{-2} M_0 \log (\epsilon_{\text{sample}}^{-1}), $ with probability $ \geq 1-\epsilon_{\text{sample}} $ over the choice of  $U_{\text{sample}}$ consisting of $M$ i.i.d. samples from $\mu_{\text{sample}} ,$  
\[ d_{TV}( \mathcal{L} (X_T^{U_{\text{sample}} } | U_{\text{sample}}), \mu) \leq \epsilon_{TV}/2. \]
\end{proposition}

\begin{proof}
Let $U_{\text{sample}}$ be a set of $M$ i.i.d. samples $x^{(1)},\cdots, x^{(M)}$ from $\mu_{\text{sample}} .$ For $ r \in \set{1, \cdots, \lfloor M/M_0\rfloor}$ Let $U_r = \set{x^{(i)} : (r-1)M_0 +1 \leq r M_0 }$ and $U_{\emptyset} = U_{\text{sample}} \setminus \bigcup_r U_r.$  Let $\nu_r$ be the uniform distribution over $U_r$ and $\nu_{\emptyset}$ be the uniform distribution over $U_{\emptyset}.$ For $m = \lfloor M/M_0\rfloor $ 
\[\nu = \frac{M_0}{M} \sum_r \nu_r + \frac{M - M_0 m }{M} \nu_{\emptyset}\]
%thus let 
%\[ \mathcal{L} (X_T^{\nu_{\text{sample}} })  = \frac{M_0}{M} \sum_r \mathcal{L} (X_T^{\nu_r })  + \frac{M - M_0 m}{M} \mathcal{L} (X_T^{\nu_{\emptyset} }) \]
%For $U,$ 
Let $ \Omega$ be the set of $U\in (\R^d)^{M_0}$ s.t. $ d_{TV}(X_T^\nu, \mu)\leq \epsilon_{TV}/2 $ with  $\nu$ being the uniform distribution over $U.$ 

Similar to the proof of \cref{prop:process init from sample disjoint case}, if we choose $M/M_0 \geq 6\epsilon_{TV}^{-2} \log (\epsilon_{\text{sample}}^{-1}), $ then with probability $ \geq 1-\epsilon_{\text{sample}},$ $\abs{\set{r: U_r\in\Omega }} \geq m(1-\epsilon_{TV}/5).$ By \cref{prop:tv distance mixture bound}, 
\begin{align*}
   d_{TV} (\mathcal{L} (X_T^{U_{\text{sample}} } | U_{\text{sample} }), \mu ) &\leq \sum_{r: U_r \in \Omega } \frac{M_0}{M} d_{TV} (  \mathcal{L} (X_T^{\nu_{r }}), \mu) + \frac{M - M_0 m(1-\epsilon_{TV}/5) }{M} \\
   &\leq \epsilon_{TV}/10 + \epsilon_{TV}^2/6 +\epsilon_{TV}/5 \leq \epsilon_{TV}/2
\end{align*}
where in the penultimate inequality, we use the definition of $ \Omega ,$ $M_0m\leq M$ and  $M-m_0 M \leq M_0 \leq \epsilon_{TV}^2 M/6.$
\end{proof}

The following proposition combined with \cref{thm:discrete mixing for cluster of distribution with close centers} implies \cref{cor:mixing of discrete chain with score error}.
\begin{proposition}\label{prop:from one distribution to mixture of distribution}
For a set $U_{\text{sample}}\subseteq \R^d$,  let $ (X_t^{U_{\text{sample}} })_t$ be a process initialized at %$\nu_{\text{sample}},$ 
the uniform distribution over
    $U_{\text{sample}}.$ %Suppose we have a partition $\mathcal{C}$ of $I.$
  Consider distributions  $\mu_C$ for $C \in \mathcal{C}.$ %and $\mu_{C,\text{sample}}.$
   Let $\mu = \sum p_C \mu_C$ with $p_C> 0$ and $\sum p_C = 1.$  Let $p_*=\min p_C.$
 Suppose there exists $T> 0, \epsilon_{TV}\in (0,1)$ 
s.t. with probability $ \geq 1-\frac{\epsilon_{\text{sample}}}{10\abs{\mathcal{C}}}$ over the choice of  $U_{C, \text{sample}}$ consisting of $M \geq M_0$ i.i.d. samples from $\mu_C,$ $d_{TV}(\mathcal{L}(X_T^{U_{C, \text{sample}}} | {U_{C, \text{sample}}} ), \mu_C) \leq \epsilon_{TV}/10.$
Then, for $M \geq  \min p_*^{-1} \set{M_0, 20 \epsilon_{TV}^{-2} \log (\abs{\mathcal{C} }\epsilon_{\text{sample}}^{-1})},$ with probability $ \geq 1-\epsilon_{\text{sample}}$ over the choice of $U_{\text{sample}}$ consisting of $M$ i.i.d. samples from $\mu,$ 
\[ d_{TV} (\mathcal{L} (X_T^{U_{\text{sample}} } | U_{ \text{sample}} ), \mu )\leq \epsilon_{TV}. \]
\end{proposition}
To remove dependency on $p_*,$ we will use the following variant of \cref{prop:from one distribution to mixture of distribution}.
\begin{proposition}\label{prop:from one distribution to mixture of distribution modified}
For a set $U_{\text{sample}}\subseteq \R^d$,  let $ (X_t^{U_{\text{sample}} })_t$ be a process initialized at %$\nu_{\text{sample}},$ 
the uniform distribution over
    $U_{\text{sample}}.$ %Suppose we have a partition $\mathcal{C}$ of $I.$
  Consider distributions  $\mu_C$ for $C \in \mathcal{C}.$ %and $\mu_{C,\text{sample}}.$
   Let $\mu = \sum p_C \mu_C$ with $p_C> 0$ and $\sum p_C = 1.$ 
  Suppose if $ p_C \geq \frac{\epsilon_{TV}}{8 \abs{\mathcal{C}}},$ there exists $T> 0, \epsilon_{TV}\in (0,1)$ 
s.t. with probability $ \geq 1-\frac{\epsilon_{\text{sample}}}{10\abs{\mathcal{C}}}$ over the choice of  $U_{C, \text{sample}}$ consisting of $M \geq M_0$ i.i.d. samples from $\mu_C,$ $d_{TV}(\mathcal{L}(X_T^{U_{C, \text{sample}}} | {U_{C, \text{sample}}}), \mu_C) \leq \epsilon_{TV}/10.$
Then, for $M \geq  (\frac{\epsilon_{TV}}{8 \abs{\mathcal{C}}})^{-1}\min  \set{M_0, 20 \epsilon_{TV}^{-2} \log (\abs{\mathcal{C} }\epsilon_{\text{sample}}^{-1})},$ with probability $ \geq 1-\epsilon_{\text{sample}}$ over the choice of $U_{\text{sample}}$ consisting of $M$ i.i.d. samples from $\mu,$ $d_{TV} (\mathcal{L} (X_T^{U_{\text{sample}} } | U_{ \text{sample}} ), \mu )\leq \epsilon_{TV} $
\end{proposition}
\begin{proof}[Proof of \cref{prop:from one distribution to mixture of distribution}]
    Since $\mu=\sum_C p_C\mu_C,$ a sample $x^{(i)}$ from $\mu$ can be drawn by first sampling  $ C^{(i)} \in \mathcal{C}$ from the distribution defined by the weights $ \set{p_C}_{C\in \mathcal{C}},$ then sample from $\mu_{C^{(i)}}.$ Consider $M$ i.i.d. samples $x^{(i)}$ using this procedure, and let $ U_C = \set{x^{(i)}: C^{(i)} = C}.$ Since $M \geq 20 p_*^{-1} \epsilon_{TV}^{-2} ,$ and $\E[\abs{U_C}] = p_C M ,$ by Chernoff's inequality and union bound, with probability $ 1-\epsilon_{\text{sample}}/2 $ over the randomness of $  U_{\text{sample}},$ the following event $\mathcal{E}_1$ holds
    \[\forall C: \abs{\frac{\abs{U_C} }{M} - p_C } \leq p_C \epsilon_{TV}/2 \]
    Suppose $\mathcal{E}_1$ holds. Then, $\frac{\abs{U_C} }{M} \geq p_C (1-\epsilon_{TV}/2) M\geq M_0.$ Thus by union bound, with probability $ 1-\epsilon_{TV}/10$ over the randomness of $  U_{\text{sample}},$ the following event $\mathcal{E}_2$ holds
    \[ \forall C: d_{TV}(\mathcal{L}(X^{U_C}_T | U_C), \mu_C) \leq \epsilon_{TV}/10 \]
    then  let $\tilde{\mu} = \sum_C \frac{\abs{U_C} }{M} \mu_C,$ by part 1 of \cref{prop:tv distance mixture bound},
    \begin{align*}
       d_{TV} (\mathcal{L}(X^{U_{\text{sample}}}_T | U_{\text{sample}}), \tilde{\mu}) = d_{TV}(\sum_C \frac{\abs{U_C} }{M} \mathcal{L}(X^{U_C}_T | U_C)   , \tilde{\mu}) \leq \sum_C \frac{\abs{U_C}}{M} \epsilon_{TV}/10 =\epsilon_{TV}/10 
    \end{align*}
    and $d_{TV} (\tilde{\mu},\mu) \leq \sum_{C} \abs{\frac{\abs{U_C} }{M} - p_C} \leq \epsilon_{TV}/2.$
    Condition on $\mathcal{E}_1$ and $\mathcal{E}_2$ both hold, which happens with probability $ 1-\epsilon_{\text{sample}},$ we have
    \begin{align*}
        d_{TV} (\mathcal{L}(X^{U_{\text{sample}}}_T | U_{\text{sample}}), \mu) &\leq d_{TV} (\mathcal{L}(X^{U_{\text{sample}}}_T | U_{\text{sample}}), \tilde{\mu})+ d_{TV}(\tilde{\mu}, \mu) \\
        &\leq \epsilon_{TV}/10 + \epsilon_{TV}/2 \leq \epsilon_{TV} 
    \end{align*}
    %With probability $  1-\epsilon_{\text{sample}}/2 $ over the randomness of 
\end{proof}
\begin{proof}[Proof of \cref{prop:from one distribution to mixture of distribution modified}]
    The proof is analogous to \cref{prop:from one distribution to mixture of distribution}. We use the same setup and will spell out the differences between the two proofs. Let $\mathcal{C}' = \set{C\in \mathcal{C}: p_C \geq \frac{\epsilon_{TV}}{8\abs{\mathcal{C}}} }.$ We redefine the event $\mathcal{E}_1$ as 
    \[\forall C \in \mathcal{C}' : \abs{\frac{\abs{U_C} }{M} - p_C } \leq p_C \epsilon_{TV}/8 \] and
    $\mathcal{E}_2$ as
     \[ \forall C \in \mathcal{C}': d_{TV}(\mathcal{L}(X^{U_C}_T | U_C), \mu_C) \leq \epsilon_{TV}/10 \]
     Let $U_\emptyset = U_{\text{sample}} \setminus \bigcup_{C\in \mathcal{C}'} C$ then \[ \frac{\abs{U_\emptyset}}{M} = \frac{\sum_{C\not\in \mathcal{C}'} \abs{U_C} }{M}\leq 1 - \sum_{C\in \mathcal{C}'} p_C (1- \epsilon_{TV}/8) \leq 1 - (1- \epsilon_{TV}/8)  (1-\epsilon_{TV}/8) \leq \epsilon_{TV}/4.\]
     Suppose $\mathcal{E}_1$ and $\mathcal{E}_2$ both hold, which occur with probability $1 -\epsilon_{\text{sample}} $ by Chernoff's inequality.
     %Let $\tilde{\mu} = \sum_{C\in \mathcal{C}'} \frac{\abs{U_C}}{M -\abs{U_\emptyset}  }\mu_C $ then  \[\abs{\frac{\abs{U_C}}{M -\abs{U_\emptyset}  }- p_C} \leq \abs{\frac{\abs{U_C}}{M -\abs{U_\emptyset}  } - \frac{\abs{U_C}}{M  } } + \abs{\frac{\abs{U_C}}{M  } - p_C}\leq \frac{\abs{U_C}}{M -\abs{U_\emptyset}  } \cdot \frac{\abs{U_\emptyset}}{M} + p_C \epsilon_{TV}/4 \]
     Let $ \tilde{\mu} =  \sum_{C\in \mathcal{C}} \frac{\abs{U_C}}{M  }\mu_C.$ %For $ C\not \in \mathcal{C'}$     \[\frac{\abs{U_C}}{M  } \]
     thus by part 1 of \cref{prop:tv distance mixture bound}
      \begin{align*}
       d_{TV} (\mathcal{L}(X^{U_{\text{sample}}}_T | U_{\text{sample}}), \tilde{\mu}) &= d_{TV}(\sum_C \frac{\abs{U_C} }{M} \mathcal{L}(X^{U_C}_T | U_C)   , \sum_{C} \frac{\abs{U_C} }{M}  \mu_C ) \\
       &\leq \sum_{C\in \mathcal{C}'} \frac{\abs{U_C}}{M} \epsilon_{TV}/10+\sum_{C\not \in\mathcal{C}' } \frac{\abs{U_C}}{M} \leq \epsilon_{TV}/10 + \epsilon_{TV}/4 \leq \epsilon_{TV}/2 
    \end{align*}
    By part 2 of \cref{prop:tv distance mixture bound}
    \[\sum_{C} \abs{\frac{\abs{U_C}}{M} - p_C} \leq \sum_{C\in \mathcal{C}'} p_C \epsilon_{TV}/8 + \sum_{C\not \in \mathcal{C}'} \max\set{\frac{\abs{U_C}}{M} 
 ,p_C} \leq \epsilon_{TV}/8 + \epsilon_{TV}/4 \]
 By triangle inequality
    \begin{align*}
        d_{TV} (\mathcal{L}(X^{U_{\text{sample}}}_T | U_{\text{sample}}), \mu) &\leq d_{TV} (\mathcal{L}(X^{U_{\text{sample}}}_T | U_{\text{sample}}), \tilde{\mu})+ d_{TV}(\tilde{\mu}, \mu) \\
        &\leq \epsilon_{TV}/2 + 3\epsilon_{TV}/8 \leq \epsilon_{TV} 
    \end{align*}
\end{proof}
\begin{comment}
\begin{proposition}
Fix $ \epsilon_{TV} , \epsilon_{\text{sample}} \in(0,1/2).$
For $x\in \R^d,$ let $(X_{nh}^x)_{n\in \N }$ be the LMC with score estimate $s$ and step size $h$ initialized at $\delta_x.$
Suppose there exists $T=Nh $ with $N\in\N$ and a partition of $I$ into $C_1, \dots, C_m$ s.t. for each $S\in \set{C_1, \dots, C_m},$ 
\[\P_{x\sim\mu}[d_{TV} (X_{T}^x , \mu_S) \leq \epsilon_{TV}] \geq p_S (1-\epsilon_{\text{sample}}) \]
Let $U_{\text{sample}}$ be a set of $M$ i.i.d. samples from $\mu$ and $ \nu_0$ be the uniform distribution over  $U_{\text{sample}}.$
Let $(X_{nh}^{\nu_0})_{n\in \N }$ be the LMC with score estimate $s$ and step size $h$ initialized at $\nu_0.$ Let $p_*=\min_i p_i.$  With probability $\geq 1 -\abs{I} \exp( -p_* (1- \epsilon_{\text{sample}}) \epsilon_{\text{sample}}^2 M/2)$  over the randomness of $U_{\text{sample}}$ %for $M\geq $
\[d_{TV} (X_{T}^{\nu_0}, \mu) \leq  (2 \abs{I} +1 )\epsilon_{TV} + (\abs{I} + 2) \epsilon_{\text{sample}}  \]
Thus, if we choose $  \epsilon_{\text{sample}} = \frac{\epsilon'_{TV} }{2 (\abs{I} + 2) }$ and $\epsilon_{TV} = \frac{\epsilon'_{TV}}{2(2 \abs{I} +1 )}$ and \[M \geq \frac{8 (\log \abs{I} + \log (1/\epsilon'_{\text{sample}})) \abs{I}^2 }{p_*^{-1}  (\epsilon'_{\text{TV}})^2 }  \geq \frac{2 (\log \abs{I} + \log (1/\epsilon'_{\text{sample}})) }{p_* (1- \epsilon_{\text{sample}}) \epsilon_{\text{sample}}^2 }   \] then with probability $\geq 1- \epsilon'_{\text{sample}}$
\[ d_{TV} (X_{T}^{\nu_0}, \mu)  \leq \epsilon'_{TV}\]

\end{proposition}
\begin{proof}
Let $\mathcal{E}_{x,C_r}$ denote the event $d_{TV}(X_{T}^x , \mu_{C_r} )\leq \epsilon_{TV}$ then 
\[\E_{x\sim \mu} [\textbf{1}[\mathcal{E}_{x,C_r}] ] \geq p_S (1-\epsilon_{\text{sample}}) . \]

Consider graph $\mathbb{H}$ over $\set{C_1,\dots, C_m}$ where there is an edge between $C_i,C_j$ if $ d_{TV}(C_i, C_j) \leq 2\epsilon_{TV}.$
Note that if $C_r, C_{r'}$ belongs to different connected components of $\mathbb{H}$ then $\mathcal{E}_{x,C_r}$ and $\mathcal{E}_{x,C_{r'}}$ are mutually exclusive events, otherwise, by triangle inequality,
\[d_{TV} (\mu_{C_r}, \mu_{C_{r'}}) \leq d_{TV}(X_{T}^x , \mu_{C_r} )+ d_{TV}(X_{T}^x , \mu_{C_{r'}} )\leq 2\epsilon_{TV} \]
thus there must be an edge in $\mathbb{H}$ between $C_r$ and $C_r',$ a contradiction. On the other hand, if $C_r$ and $C_{r'}$  belongs to the same connected components of $\mathbb{H}$ then there exists a path $ C_r:= C_{r_0}, C_{r_1}, \dots, C_{r_k} =C_{r'}$ s.t. $d_{TV}(C_{r_i}, C_{r_{i+1}}) \leq 2\epsilon_{TV},$ thus by triangle inequality
\[d(C_r, C_{r'}) \leq \sum_{i=0}^{k-1} d_{TV}(C_{r_i}, C_{r_{i+1}}) \leq 2 k \epsilon_{TV} \leq 2 \abs{I} \epsilon_{TV} \]

Let $\hat{C}_1, \cdots, \hat{C}_{\hat{m}}$ be the connected components of $\mathbb{H}.$ %Since we can arbitrarily relabel the $C_r$'s, we can assume s.l.o.g. assume that $C_r \in \hat{C}_r\forall r\in [\hat{m}].$ 

We abuse notation and use $\hat{C}_{\hat{r}} $ to denote $\bigcup_{C_{r'}\in \hat{C}_{\hat{r}}} C_{r'}\subseteq I.$ Note  $\mu_{\hat{C}_{\hat{r}}}$ is a linear combination of $\mu_{C_{r'}}$ for $C_{r'}\in \hat{C}_{\hat{r}}$ i.e. $p_{\hat{C}_{\hat{r}}} \mu_{\hat{C}_{\hat{r}}} = \sum_{C_{r'}\in \hat{C}_{\hat{r}}} p_{C_{r'}} \mu_{C_{r'}},$ thus, by triangle inequality, for any $C_{r'}\in \hat{C}_{\hat{r}}$
\[d_{TV}(\mu_{C_{r'}}, \mu_{\hat{C}_{\hat{r}}}) \leq \max_{C_{\bar{r} } \in \hat{C}_{\hat{r}}} d_{TV} (\mu_{C_r},  \mu_{C_{\bar{r} }}) \leq  2 \abs{I} \epsilon_{TV}  \]
Let $\hat{\mathcal{E}}_{x, \hat{C}_{\hat{r}}}$ be the union of the events $ \mathcal{E}_{x, C_{r'}}$ for $C_{r'} \in \hat{C}_{\hat{r}},$ then $\textbf{1} [\hat{\mathcal{E}}_{x, \hat{C}_{\hat{r}}}]=\max_{C_{r'}\in \hat{C}_{\hat{r}}} \textbf{1} [\mathcal{E}_{x,C_{r'}}],$ thus
\begin{align*}
  \E_{x\sim \mu} [\textbf{1} [\hat{\mathcal{E}}_{x, \hat{C}_{\hat{r}}}] ] &= \int \mu(x) \textbf{1} [\mathcal{E}_{x, \hat{C}_{\hat{r}}}]dx
  \geq \int\left( \sum_{C_{r'}\in\hat{C}_{\hat{r}}}   p_{C_{r'}} \mu_{C_{r'}} \right) \max_{C_{r'}\in \hat{C}_{\hat{r}}} \textbf{1} [\mathcal{E}_{x,C_{r'}}] dx\\
  &\geq \int \sum_{C_{r'}\in\hat{C}_{\hat{r}}}   p_{C_{r'}} \mu_{C_{r'}} \textbf{1} [\mathcal{E}_{x,C_{r'}}] dx
  \geq \sum_{C_{r'}\in\hat{C}_{\hat{r}}}   p_{C_{r'}} \E_{\mu_{C_{r'}}}[\textbf{1} [\mathcal{E}_{x,C_{r'}}] ]\\
  &\geq (1-\epsilon_{\text{sample}}) \sum_{C_{r'}\in\hat{C}_{\hat{r}}}   p_{C_{r'}} = (1-\epsilon_{\text{sample}}) p_{\hat{C}_{\hat{r}}}.
\end{align*}
If $ \hat{\mathcal{E}}_{x, \hat{C}_{\hat{r}}}$ holds then there exists $C_{r}\in \hat{C}_{\hat{r}}$ s.t. $d_{TV} (X_T^x, C_{r}) \leq \epsilon_{TV},$ thus by triangle inequality 
\[d_{TV}(X_T^x, \mu_{\hat{C}_{\hat{r}}}) \leq d_{TV} (X_T^x, \mu_{C_{r}}) + d_{TV}(\mu_{C_{r}}, \mu_{\hat{C}_{\hat{r}}})  \leq (2\abs{I} +1)\epsilon_{TV} \]
Lastly, the event $ \hat{\mathcal{E}}_{x, \hat{C}_{\hat{r}}}$ and $ \hat{\mathcal{E}}_{x, \hat{C}_{\hat{r}'}}$ are mutually exclusive for $ \hat{r}\neq\hat{r}',$ since for any $C_r \in \hat{C}_{\hat{r}} $ and $C_{r'} \in \hat{C}_{\hat{r'}} $, $\mathcal{E}_{x,C_r}$ and $\mathcal{E}_{x,C_{r'}}$ are mutually exclusive.

Let $U_{\hat{r}}$ denote the set of $x\in U_{\text{sample}} $ s.t. $ \hat{\mathcal{E}}_{x,\hat{C}_{\hat{r}}}$ holds and $ M_{\hat{r}}= \abs{U_{\hat{r}}} =\sum_{x\in U_{\text{sample}}} \textbf{1}[\hat{\mathcal{E}}_{x,\hat{C}_{\hat{r}}}].$ Note that $U_{\hat{r}}$'s are disjoint. %denote the number of $x$ in $U_{\text{sample}}$ s.t. $ \hat{\mathcal{E}}_{x,\hat{C}_{\hat{r}}}$ holds. 
By Chernoff's bound
%\[\P[\abs{M_{\hat{r}}/M -p_S}  ]\]
\[\P[ M_{\hat{r}} \geq p_{\hat{C}_{\hat{r}}} (1- \epsilon_{\text{sample}})^2 M ] \geq 1- \exp(-p_{\hat{C}_{\hat{r}}} (1- \epsilon_{\text{sample}})^3 M/2) \]
By union bound over all $\hat{C}_{\hat{r}},$ let $\hat{E}$ be the event $\forall \hat{r}: M_{\hat{r}} \geq p_{\hat{C}_{\hat{r}}} (1- \epsilon_{\text{sample}})^2 M$ then
\[\P[ \hat{E}] \geq 1- \sum_{\hat{r}} \exp(-p_{\hat{C}_{\hat{r}}} (1- \epsilon_{\text{sample}})\epsilon_{\text{sample}}^2  M/2) \geq 1 -\abs{I} \exp( -p_* (1- \epsilon_{\text{sample}}) \epsilon_{\text{sample}}^2 M/2)  \]
where we recall that $p_*=\min p_i.$

Suppose $\hat{E}$ occurs. Since $\sum_{\hat{r}} M_{\hat{r}}\leq M,$  $ M_{\hat{r}} - p_{\hat{C}_{\hat{r}}} (1- \epsilon_{\text{sample}})^2 M  \leq M  - \sum_{\hat{r}'\neq \hat{r}} p_{\hat{C}_{\hat{r}'}} (1- \epsilon_{\text{sample}})^2 M - p_{\hat{C}_{\hat{r}}} (1- \epsilon_{\text{sample}})^2 M = M( 1- (1- \epsilon_{\text{sample}})^2) \leq 2M \epsilon_{\text{sample}}. $

Let $U_{\emptyset} =U_{\text{sample}} \setminus \bigcup_{\hat{r}}  U_{\hat{r}} $ then $\abs{U_{\emptyset}} \leq M - \sum_{\hat{r}} p_{\hat{C}_{\hat{r}}} (1- \epsilon_{\text{sample}})^2 M\leq M(1- (1- \epsilon_{\text{sample}})^2)  \leq 2M \epsilon_{\text{sample}}.$ Note that $\mathcal{L}(X_T^{\nu_0}) = \frac{1}{M}  \sum_{x\in U_{\text{sample}}} \mathcal{L}(X_T^x)$ where $\mathcal{L}(X)$ refers to the law of the random variable $X.$ Thus, with $ \tilde{\mu} := \sum_{\hat{r}} \frac{\abs{U_{\hat{r}}} }{M} \mu_{\hat{C}_{\hat{r}}} + \frac{\abs{U_{\emptyset} }}{M}\mu$,  we can apply part 1 of \cref{prop:tv distance mixture bound}
\begin{align*}
    d_{TV}(X_T^{\nu_0},  \tilde{\mu}) &\leq M^{-1} \left ( \sum_{\hat{r}} \sum_{x\in U_{\hat{r}}} d_{TV}(X_T^x, \mu_{\hat{C}_{\hat{r}}} ) + \sum_{x\in U_{\emptyset} } d_{TV} (X_T^x, \mu)\right)\\
    &\leq M^{-1} ( (2 \abs{I} +1 )\epsilon_{TV} (M - \abs{U_{\emptyset}}) +   \abs{U_{\emptyset}}) \\
    &\leq (2 \abs{I} +1 )\epsilon_{TV} + 2 \epsilon_{\text{sample}}
\end{align*}
Next, note that $\mu=\sum_{\hat{r}} p_{\hat{C}_{\hat{r}}} \mu_{\hat{C}_{\hat{r}}} $ and $\tilde{\mu} =\sum_{\hat{r}} (\frac{\abs{U_{\hat{r}}} }{M} +  p_{\hat{C}_{\hat{r}}} \frac{\abs{U_{\emptyset} }}{M} ) \mu_{\hat{C}_{\hat{r}}} .$  Part 2 of \cref{prop:tv distance mixture bound} gives
\begin{align*}
   d_{TV}( \tilde{\mu}, \mu) &\leq \frac{1}{2} \sum_{\hat{r}} \abs{p_{\hat{C}_{\hat{r}}} - (\frac{\abs{U_{\hat{r}}} }{M} +  p_{\hat{C}_{\hat{r}}} \frac{\abs{U_{\emptyset} }}{M} ) } =  \frac{1}{2} \sum_{\hat{r}} \abs{p_{\hat{C}_{\hat{r}}} (1 - \frac{\abs{U_{\emptyset} }}{M} ) -\frac{\abs{U_{\hat{r}}} }{M}  } \\
   &\leq \frac{1}{2} \sum_{\hat{r}} \max \set{p_{\hat{C}_{\hat{r}}}  -  \frac{\abs{U_{\hat{r}}} }{M} ,\frac{\abs{U_{\hat{r}}} }{M}-  p_{\hat{C}_{\hat{r}}} (1-\epsilon_{\text{sample}} )^2 }\\
   &\leq  \frac{1}{2} \sum_{\hat{r}} \max \set{p_{\hat{C}_{\hat{r}}}  2  \epsilon_{\text{sample}}  , 2  \epsilon_{\text{sample}}} \leq \abs{I}  \epsilon_{\text{sample}}
\end{align*}
thus by triangle inequality
\[d_{TV} (X_T^{\nu_0}, \mu) \leq  d_{TV}(X_T^{\nu_0},  \tilde{\mu})  + d_{TV}( \tilde{\mu}, \mu) \leq  (2 \abs{I} +1 )\epsilon_{TV} + (\abs{I} + 2) \epsilon_{\text{sample}} \]
\end{proof}
\end{comment}
%\input{initialization}
%\input{gradient error}
%\input{perturbation and drift}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

